Teaching Transformers Causal Reasoning through Axiomatic Training

For text-based AI systems to interact in the real world, causal reasoning is an essential skill. Since active interventions are costly, we study to what extent a system can learn causal reasoning from symbolic demonstrations of causal axioms. Specifically, we present an axiomatic training method where the system learns from multiple demonstrations of a causal axiom (or rule), rather than incorporating the axiom as an inductive bias or inferring it from data values. A key question is whether the system would learn to generalize from the axiom demonstrations to more complex scenarios. Our results, based on applying axiomatic training to learn the transitivity axiom and d-separation rule, indicate that such generalization is possible. To avoid data contamination issues, we start with a 67 million parameter transformer model and train it from scratch. On both tasks, we find that a model trained on linear causal chains (along with some noisy variations) can generalize well to complex graphs, including longer causal chains, causal chains with reversed order, and graphs with branching.To handle diverse text inputs, the same method is extended to finetune language models. Finetuning Llama-3-8B-Instruct model on our axiomatic data leads to significant gains on causal benchmarks such as Corr2Cause and CLEAR, in some cases providing state-of-the-art performance surpassing GPT-4.

==> sections/ethical_consideration.tex <==
\section*{Ethical Impact and Reproducibility}
%\new{
% \textit{Limitations and Future work} While our work provides a potential way of improving fundamental reasoning capabilities of language models, the current work is restricted to synthetic tasks. Future work could build upon it to directly relate to real world problems. More axioms of causality/logic could also be incorporated. 

\textit{Ethical Statement.} All datasets used in our work will be made publicly available for evaluation of future iterations of models. We made best efforts to compare against contemporary models in a fair manner. There may be no direct harmful impact, especially considering our work focuses on a synthetic symbolic setting. However, since LLMs may be used in our approach, suitable prudence may be necessary to avoid ill-effects in applications.

\textit{Reproducibility.} Our methods are fairly straightforward. Most implementation details are already included in our paper. We will release our code publicly on acceptance.
